On Usage of Non-Volatile Memory as Primary Storage for Database Management Systems

This paper explores the implications of employing non-volatile memory (NVM) as primary storage for a data base management system (DBMS). We investigate the modifications necessary to be applied on top of a traditional relational DBMS to take advantage of NVM features. As a case study, we modify the storage engine (SE) of PostgreSQL enabling efficient use of NVM hardware. We detail the necessary changes and challenges such modifications entail and evaluate them using a comprehensive emulation platform. Results indicate that our modified SE reduces query execution time by up to 45% and 13% when compared to disk and NVM storage, with average reductions of 19% and 4%, respectively. Detailed analysis of these results shows that while our modified SE is able to access data more efficiently, data is not close to the processing units when needed for processing, incurring long latency misses that hinder the performance. To solve this, we develop a general purpose library that employs helper threads to prefetch data from NVM hardware via a simple API. Our library further improves query execution time for our modified SE when compared to disk and NVM storage by up to 54% and 17%, with average reductions of 23% and 8%, respectively.

==> References.tex <==

\bibitem{abraham2013scuba}
Abraham L, Allen J, Barykin O, Borkar V, Chopra B, Gerea C, Merl D, Metzler J, Reiss D, Subramanian S, Wiener JL.: Scuba: diving into data at facebook. Proceedings of the VLDB Endowment. \textbf{6}(11), 1057--1067 (2013)

%\bibitem{baulier1998datablitz}
%Baulier J, Bohannon P, Gogate S, Joshi S, Gupta C, Khivesera A, Korth HF, McIlroy P, Miller J, Narayan PP, Nemeth M. DataBlitz: A High Performance Main-Memory Storage Manager. In: Proceedings of the 24th International Conference on Very Large Data Bases. 1998, p. 701

\bibitem{barber2011blink}
Barber R, Bendel P, Czech M, Draese O, Ho F, Hrle N, Idreos S, Kim MS, Koeth O, Lee JG, Li TT, Lohman G, Morfonios , Mueller R, Murthy K, Pandis I, Qiao L, Raman V, Szabo S, Sidle R, Stolze K.: Blink: Not Your Father\textquotesingle s Database!. In: Proceedings of International Workshop on Business Intelligence for the Real-Time Enterprise, pp. 1--22 (2011)


\bibitem{farber2012sap}
F\"{a}rber F, Cha SK, Primsch J, Bornh\"{o}vd C, Sigg S, Lehner W.: SAP HANA database: data management for modern business applications. ACM Sigmod Record.  \textbf{40}(4), 45--51 (2012)

\bibitem{lindstrom2013ibm}
Lindstr\"{o}m J, Raatikka V, Ruuth J, Soini P, Vakkila K.: IBM solidDB: In-Memory Database Optimized for Extreme Speed and Availability. IEEE Data Eng. Bull. \textbf{36}(2), 14--20 (2013)

\bibitem{PeletonLink}
Peloton Database Management System. Published at http://pelotondb.org (2019)

\bibitem{pavlo2017self}
Pavlo A, Angulo G, Arulraj J, Lin H, Lin J, Ma L, Menon P, Mowry TC, Perron M, Quah I, Santurkar S, Tomasic A, Toor S, Aken D.V, Wang Z, Wu Y, Xian R, Zhang T.: Self-Driving Database Management Systems. In: Proceedings of Biennial Conference on Innovative Data Systems Research (CIDR) (2017)

\bibitem{larson2011sql}
Larson P\r{A}, Clinciu C, Hanson EN, Oks A, Price SL, Rangarajan S, Surna A, Zhou Q.: SQL server column store indexes. In: Proceedings of the ACM SIGMOD International Conference on Management of Data, pp. 1177--1184 (2011)

%\bibitem{lehman1986study}
%Lehman TJ, Carey MJ. A study of index structures for main memory database management systems. In: Proceedings of the 12th International Conference on Very Large Data Bases. 1986, 294--303

\bibitem{zhang2016reducing}
Zhang H, Andersen DG, Pavlo A, Kaminsky M, Ma L, Shen R.: Reducing the storage overhead of main-memory OLTP databases with hybrid indexes. In: Proceedings of the International Conference on Management of Data, pp. 1567--1581 (2016)

\bibitem{ongaro2011fast}
Ongaro D, Rumble SM, Stutsman R, Ousterhout J, Rosenblum M.: Fast crash recovery in RAMCloud. In: Proceedings of the Twenty-Third ACM Symposium on Operating Systems Principles (SOSP), pp. 29--41 (2011)

%\bibitem{lehman1987recovery}
%Lehman TJ, Carey MJ. A recovery algorithm for a high-performance memory-resident database system. In: Proceedings of the 1987 ACM SIGMOD international conference on Management of data. 1987, 104--117

\bibitem{diaconu2013hekaton}
Diaconu C, Freedman C, Ismert E, Larson PA, Mittal P, Stonecipher R, Verma N, Zwilling M.: Hekaton: SQL server's memory-optimized OLTP engine. In: Proceedings of the ACM SIGMOD International Conference on Management of Data, pp. 1243--1254 (2013)

\bibitem{lee2001single}
Lee I, Yeom HY.: A single phase distributed commit protocol for main memory database systems. In: Proceedings of Parallel and Distributed Processing Symposium, (2002)

\bibitem{debrabant2014prolegomenon}
DeBrabant J, Arulraj J, Pavlo A, Stonebraker M, Zdonik S, Dulloor S.: A prolegomenon on OLTP database systems for non-volatile memory. In International Workshop on Accelerating Data Management Systems Using Modern Processor and Storage Architectures. (2014)

\bibitem{driskill2010latest}
Driskill-Smith A.: Latest advances and future prospects of STT-RAM. In Non-Volatile Memories Workshop. 11--13, (2010)

\bibitem{mandelman2002challenges}
Mandelman JA, Dennard RH, Bronner GB, DeBrosse JK, Divakaruni R, Li Y, Radens CJ.: Challenges and future directions for the scaling of dynamic random-access memory (DRAM). IBM Journal of Research and Development. \textbf{46}(2.3), 187--212 (2002)

\bibitem{melnik2010dremel}
Melnik S, Gubarev A, Long JJ, Romer G, Shivakumar S, Tolton M, Vassilakis T.: Dremel: interactive analysis of web-scale datasets. Proceedings of the VLDB Endowment.  \textbf{3}(1--2) 330--339 (2010)

\bibitem{plattner2011sanssoucidb}
Plattner H.: SanssouciDB: An In-Memory Database for Processing Enterprise Workloads. In: Proceedings of Datenbanksysteme f\"{u}r Business, Technologie und Web (BTW), pp. 2--21 (2011)

\bibitem{sikka2012efficient}
Sikka V, F\"{a}rber F, Lehner W, Cha SK, Peh T, Bornh\"{o}vd C.: Efficient transaction processing in SAP HANA database: the end of a column store myth. In: Proceedings of the 2012 ACM SIGMOD International Conference on Management of Data, pp. 731--742 (2012)

\bibitem{arulraj2017build}
Arulraj J, Pavlo A.: How to Build a Non-Volatile Memory Database Management System. In: Proceedings of the 2017 ACM International Conference on Management of Data, pp. 1753--1758 (2017)

\bibitem{qureshi2009scalable}
Qureshi MK, Srinivasan V, Rivers JA.: Scalable high performance main memory system using phase-change memory technology. In: Proceedings of the 36th annual international symposium on Computer architecture (ISCA), pp. 24--33 (2009)

\bibitem{andrei2017sap}
Andrei M, Lemke C, Radestock G, Schulze R, Thiel C, Blanco R, Meghlan A, Sharique M, Seifert S, Vishnoi S, Booss D, Peh T, Schreter I, Thesing W, Wagle  M, Willhalm T.: SAP HANA adoption of non-volatile memory. Proceedings of the VLDB Endowment. \textbf{10}(12), 1754--1765 (2017)

\bibitem{raoux2008phase}
Raoux S, Burr GW, Breitwisch MJ, Rettner CT, Chen YC, Shelby RM, Salinga M, Krebs D, Chen SH, Lung HL, Lam CH.: Phase-change random access memory: A scalable technology. IBM Journal of Research and Development. \textbf{52}(4.5), 465--479 (2008)

\bibitem{strukov2008missing}
Strukov DB, Snider GS, Stewart DR, Williams RS.: The missing memristor found. nature. \textbf{453}(7191), 80--83 (2008)


\bibitem{arulraj2015let}
Arulraj J, Pavlo A, Dulloor SR.: Let's talk about storage \& recovery methods for non-volatile memory database systems. In: Proceedings of the 2015 ACM SIGMOD International Conference on Management of Data, pp. 707--722 (2015)

\bibitem{chang2012limits}
Chang J, Ranganathan P, Mudge T, Roberts D, Shah MA, Lim KT.: A limits study of benefits from nanostore-based future data-centric system architectures. In: Proceedings of the 9th conference on Computing Frontiers (CF), pp. 33--42 (2012)

\bibitem{hagmann2002real}
Hagmann R, Skeen MD.: Real-time query optimization in a decision support system. United States patent US 6,338,055. (2002)

\bibitem{shim2002past}
Shim JP, Warkentin M, Courtney JF, Power DJ, Sharda R, Carlsson C.: Past, present, and future of decision support technology. Decision support systems. \textbf{33}(2), 111--126 (2002)

\bibitem{chaudhuri2001database}
Chaudhuri S, Dayal U, Ganti V.: Database technology for decision support systems. Computer. \textbf{34}(12), 48--55 (2001)

\bibitem{DBRanking}
DB-Engines Ranking of Relational DBMS. Published at https://db-engines.com/en/ranking (2019)

\bibitem{council2008tpc}
Transaction Processing Performance Council. TPC-H benchmark specification. Published at http://www.tpc.org/tpch/ (2008)

\bibitem{perez2010non}
Perez T, De Rose CA.: Non-volatile memory: Emerging technologies and their impacts on memory systems. Technical Report, Porto Alegre (2010)

\bibitem{wang2013low}
Wang KL, Alzate JG, Amiri PK.: Low-power non-volatile spintronic memory: STT-RAM and beyond. Journal of Physics D: Applied Physics. \textbf{46}(7), 074003 (2013)


\bibitem{mittal2016survey}
Mittal S, Vetter JS.: A survey of software techniques for using non-volatile memories for storage and main memory systems. IEEE Transactions on Parallel and Distributed Systems. \textbf{27}(5), 1537--1550 (2016)

\bibitem{arulraj2016write}
Arulraj J, Perron M, Pavlo A.: Write-behind logging. Proceedings of the VLDB Endowment. \textbf{10}(7), 337--348 (2016)

\bibitem{oukid2014sofort}
Oukid I, Booss D, Lehner W, Bumbulis P, Willhalm T.: SOFORT: A hybrid SCM-DRAM storage engine for fast data recovery. In: Proceedings of the Tenth International Workshop on Data Management on New Hardware (DaMoN), (2014)

\bibitem{chatzistergiou2015rewind}
Chatzistergiou A, Cintra M, Viglas SD.: Rewind: Recovery write-ahead system for in-memory non-volatile data-structures. Proceedings of the VLDB Endowment. \textbf{8}(5), 497--508 (2015)

\bibitem{huang2012register}
Huang Y, Liu T, Xue CJ.: Register allocation for write activity minimization on non-volatile main memory for embedded systems. Journal of Systems Architecture. \textbf{58}(1), 13--23 (2012)

\bibitem{oukid2015instant}
Oukid I, Lehner W, Kissinger T, Willhalm T, Bumbulis P.: Instant Recovery for Main Memory Databases. In: Proceedings of Biennial Conference on Innovative Data Systems Research (CIDR), (2015)

\bibitem{chakrabarti2014atlas}
Chakrabarti DR, Boehm HJ, Bhandari K.: Atlas: Leveraging locks for non-volatile memory consistency. In: Proceedings of ACM International Conference on Object Oriented Programming Systems Languages \& Applications (OOPSLA), pp. 433--452 (2014)

\bibitem{zhang2015study}
Zhang Y, Swanson S.: A study of application performance with non-volatile main memory. In: Proceedings of 31st IEEE Symposium on Mass Storage Systems and Technologies (MSST), pp. 1--10 (2015)

\bibitem{viglas2014write}
Viglas SD.: Write-limited sorts and joins for persistent memory. Proceedings of the VLDB Endowment. \textbf{7}(5), 413--424 (2014)

\bibitem{zhou2009durable}
Zhou P, Zhao B, Yang J, Zhang Y.: A durable and energy efficient main memory using phase change memory technology. In: Proceedings of the 36th annual international symposium on Computer architecture (ISCA), pp. 14--23 (2009)

\bibitem{3DXPoint}
Intel and Micron. 3D XPoint Technology. https://www.micron.com/products/advanced-solutions/3d-xpoint-technology (2019)

\bibitem{intel2016architecture}
Intel. 2016. Architecture Instruction Set Extensions Programming Reference. Intel Corporation. (2016)

\bibitem{dulloor2014system}
Dulloor SR, Kumar S, Keshavamurthy A, Lantz P, Reddy D, Sankaran R, Jackson J.: System software for persistent memory. In: Proceedings of the Ninth European Conference on Computer Systems, p. 15 (2014)

\bibitem{githubPMFS}
Intel. 2014. Linux-pmfs. https://github.com/linux-pmfs/pmfs (2014)

\bibitem{kimura2015foedus}
Kimura H.: FOEDUS: OLTP Engine for a Thousand Cores and NVRAM. In: Proceedings of the ACM SIGMOD International Conference on Management of Data, pp. 691--706 (2015)

\bibitem{huang2014nvram}
Huang J, Schwan K, Qureshi MK.: NVRAM-aware logging in transaction systems. Proceedings of the VLDB Endowment. \textbf{8}(4), 389--400 (2014)

\bibitem{schindler2002track}
Schindler J, Griffin JL, Lumb CR, Ganger GR.: Track-Aligned Extents: Matching Access Patterns to Disk Drive Characteristics. In: Proceedings of the 1st USENIX Conference on File and Storage Technologies (FAST), pp. 259--274 (2002)

\bibitem{debrabant2013anti}
DeBrabant J, Pavlo A, Tu S, Stonebraker M, Zdonik S.: Anti-caching: A new approach to database management system architecture. Proceedings of the VLDB Endowment. \textbf{6}(14), 1942--1953 (2013)

%\bibitem{garcia1992main}
%Garcia-Molina H, Salem K. Main memory database systems: An overview. IEEE Transactions on knowledge and data engineering, 1992, 4(6): 509--16

\bibitem{pelley2014memory}
Pelley S, Chen PM, Wenisch TF.: Memory persistency. In: Proceedings of ACM/IEEE 41st International Symposium on Computer Architecture (ISCA), pp. 265--276 (2014)

\bibitem{momjian2001postgresql}
Momjian B.: PostgreSQL: introduction and concepts. New York: Addison-Wesley (2001)

\bibitem{neumann2015fast}
Neumann T, M\"{u}hlbauer T, Kemper A.: Fast serializable multi-version concurrency control for main-memory database systems. In: Proceedings of the ACM SIGMOD International Conference on Management of Data, pp. 677--689 (2015)

\bibitem{PostgreSQLDocBook}
The PostgreSQL Global Development Group. PostgreSQL 9.0.22 Documentation. (2015)

\bibitem{gao2011pcmlogging}
Gao S, Xu J, He B, Choi B, Hu H.: PCMLogging: reducing transaction logging overhead with PCM. In: Proceedings of the 20th ACM international conference on Information and knowledge management, pp. 2401--2404 (2011)

\bibitem{son2017log}
Son Y, Kang H, Yeom HY, Han H.: A log-structured buffer for database systems using non-volatile memory. In: Proceedings of the Symposium on Applied Computing (SAC), pp. 880--886 (2017)

\bibitem{annavaram2001data}
Annavaram M, Patel JM, Davidson ES. Data prefetching by dependence graph precomputation. In: Procedings of 28th Annual International Symposium on Computer Architecture (ISCA), pp. 52--61 (2001)

\bibitem{jung2006helper}
Jung C, Lim D, Lee J, Solihin Y.: Helper thread prefetching for loosely-coupled multiprocessor systems. In: Proceedings of 20th International Parallel and Distributed Processing Symposium, (2006)

\bibitem{pelley2013storage}
Pelley S, Wenisch TF, Gold BT, Bridge B.: Storage management in the NVRAM era. Proceedings of the VLDB Endowment. \textbf{7}(12), 121--132 (2013)

\bibitem{johnson2009shore}
Johnson R, Pandis I, Hardavellas N, Ailamaki A, Falsafi B.: Shore-MT: a scalable storage manager for the multicore era. In: Proceedings of the 12th International Conference on Extending Database Technology: Advances in Database Technology (EDBT), pp. 24--35 (2009)

\bibitem{fang2011high}
Fang R, Hsiao HI, He B, Mohan C, Wang Y.: High performance database logging using storage class memory. In: Proceedings of IEEE 27th International Conference on Data Engineering, pp. 1221--1231 (2011)

\bibitem{wang2014scalable}
Wang T, Johnson R.: Scalable logging through emerging non-volatile memory. Proceedings of the VLDB Endowment. \textbf{7}(10), 865--876 (2014)

\bibitem{RankingLink}
DB-Engines Ranking - popularity ranking of database management systems. Published at https://db-engines.com/en/ranking (2019)

\bibitem{kamruzzaman2011inter}
Kamruzzaman M, Swanson S, Tullsen DM.: Inter-core prefetching for multicore processors using migrating helper threads. In: Proceedings of the sixteenth international conference on Architectural support for programming languages and operating systems (ASPLOS), pp. 393--404 (2011)

\bibitem{kim2002design}
Kim D, Yeung D.: Design and evaluation of compiler algorithms for pre-execution. In: Proceedings of the 10th international conference on Architectural support for programming languages and operating systems (ASPLOS), pp. 159--170  (2002)
%\vspace*{-1mm}

\bibitem{collins2001dynamic}
Collins JD, Tullsen DM, Wang H, Shen JP.: Dynamic speculative precomputation. In: Proceedings of the 34th annual ACM/IEEE international symposium on Microarchitecture (MICRO), pp. 306--317 (2001)




==> case-study.tex <==
\section{A Case Study: P\MakeLowercase{ostgre}SQL}
\label{sec:CaseStudy}
\noindent PostgreSQL is an open source object-relational database system. It is fully atomicity, consistency, isolation, durability (ACID) 
compliant and runs on all major operating systems including Linux \cite{momjian2001postgresql}. In this section, we study the 
storage engine (SE) of PostgreSQL and apply necessary changes to make it NVM-aware. We first describe the read-write architecture 
of PostgreSQL and then explain our modifications.



\subsection{Read-Write Architecture of PostgreSQL}

Fig.~\ref{Fig3a} shows the original PostgreSQL architecture from the perspective of read and write file operations. 
The left column in the figure shows the operations performed by different software layers of PostgreSQL, while the right column 
shows the corresponding data movement activities. Note that in Fig.~\ref{Fig3a} we assume the disk has already been replaced 
by NVM hardware with PMFS as the file system. However, the same behavior would be expected using a regular disk and a traditional 
FS, since PostgreSQL heavily relies on file I/O for read and write operations and the file I/O APIs in PMFS are the same as those 
in a traditional FS.

The PostgreSQL server calls the services of the  \textit{Buffer Layer} which is responsible for maintaining an 
internal buffer cache. The buffer cache is used to keep a copy of the requested page which is read from the 
storage. Copies are kept in the cache as long as they are needed. If there is no free
slot available for a newly requested page then a replacement policy is used to select a victim. 
The victim is evicted from the buffer cache and if it is 
a dirty page, then it is also flushed back to the permanent storage.

Upon receiving a new request to read a page from storage, the \textit{Buffer Layer} finds a free buffer cache slot 
and gets a pointer to it. The free buffer slot and corresponding pointer are shown in Fig.~\ref{Fig3a} as \textit{Pg Buffer} and \textit{PgBufPtr}, respectively. The \textit{Buffer Layer} then passes the pointer to the \textit{File Layer}. Eventually, the \textit{File Layer} of PostgreSQL invokes the file read and write system calls implemented by the 
underlying FS. 

For a read operation, PMFS copies the data block from NVM to a kernel buffer and then the kernel copies the requested 
data block to an internal buffer slot pointed by \textit{PgBufPtr}. In the same way, two copies are made for write operation but in the opposite direction.

Hence, the SE of original PostgreSQL incurs two copy operations for each miss in the internal buffer cache. This is 
likely to become a big overhead for databases running queries on large datasets. However, since PMFS can map the entire NVM address space into the kernel's virtual address space~\cite{dulloor2014system}, the copy overhead can be avoided by making modifications in the SE. We apply these modifications in two incremental steps as described in 
the following subsections.

\subsection{SE1: Using Memory Mapped I/O}
In the first step towards leveraging the features of NVM, we replace the \textit{File Layer} of PostgreSQL by a 
new layer named \textit{MemMapped Layer}. As shown in Fig. \ref{Fig3b}, this layer still receives a pointer 
to a free buffer slot from the \textit{Buffer Layer}, but instead of using the file I/O interface, it uses the memory 
mapped I/O interface of PMFS. We term this storage engine \textit{SE1}.

\noindent\textbf{Read Operation:} When accessing a file for a read operation, we first open the file using the \verb+open()+ 
system call, same as in original PostgreSQL. Additionally, we create a mapping of the file using \verb+mmap()+. 
Since we are using PMFS, \verb+mmap()+ returns a pointer to the mapping of the file stored in NVM. The implementation of \verb+mmap()+ by PMFS provides the application with direct access to mapped pages of files residing in NVM.

As a result, we do not need to make an intermediate copy of the requested page from NVM into kernel buffers. We can 
directly copy the requested page into internal buffers of PostgreSQL by using an implicit \verb+memcpy()+ as shown in Fig. \ref{Fig3b}. When all requested operations on a given file are completed and it is not needed anymore, 
the file can be closed. Upon closing a file, we delete the mapping of the file by calling the \verb+munmap()+ function. 

\noindent\textbf{Write Operation:} The same approach as in the read operation is used for writing data into a file. The file to be modified is first opened and a mapping is created using \verb+mmap()+. The data to be written into the file is copied 
directly from internal buffers of PostgreSQL into NVM using \verb+memcpy()+.

An SE with the above-mentioned modifications does not create an intermediate copy of the data in kernel buffers. Hence 
we reduce the overhead to one copy operation for each miss in the internal buffer cache of PostgreSQL. 

\subsection{SE2: Direct Access to Mapped Files}
In the second step of modifications to the SE, we replace the \textit{MemMapped Layer} of SE1 by 
the \textit{PtrRedirection Layer} as shown in Fig.~\ref{Fig3c}. Unlike the \textit{MemMapped Layer}, 
the \textit{PtrRedirection Layer} in SE2 receives the pointer to \textit{PgBufPtr} (i.e \textit{P2PgBufPtr}), which itself points to a free slot of the buffer cache. In other words, \textit{PtrRedirection Layer} receives a pointer to a pointer from the \textit{Buffer Layer}.

\noindent\textbf{Read Operation:} When accessing a file for a read operation, we first open the file using \verb+open()+ system call, same as in original PostgreSQL and SE1. Additionally, we also create a mapping of the file using \verb+mmap()+. Originally \textit{PgBufPtr} points to a free slot in the 
internal buffer cache. Since \verb+mmap()+ makes the NVM mapped address space visible to the calling process, the \textit{PtrRedirection Layer} simply redirects the \textit{PgBufPtr} to point to the corresponding address of the file residing in NVM. Pointer redirection in case of a read operation is shown by a black dashed arrow with the ``Read'' label in Fig.~\ref{Fig3c}.

As a result of pointer redirection and the visibility of the NVM address space enabled by PMFS, we incur no copy 
overhead for read operations. This can represent a significant improvement since read operations are predominant in queries that operate on large datasets.

\noindent\textbf{Write Operation:} PMFS provides direct write access for files residing in NVM. 
However, it does not manage the data consistency in memory mapped operations and leaves the responsibility 
to the application \cite{dulloor2014system} - i.e., PostgreSQL.


PostgreSQL is an ACID compliant DBMS which uses 
multi-version concurrency control (MVCC) \cite{neumann2015fast}
%MultiVersion Concurrency Control (MVCC) 
to maintain data consistency.
Under MVCC, concurrent executing transactions see a snapshot of the data at a particular instant in time, 
regardless of the current state of the underlying data. This provides data consistency and transaction isolation \cite{PostgreSQLDocBook}. 

To keep the consistency model of PostgreSQL unaltered and functionally correct,
SE2 performs two actions before modifying the 
actual content of the page and marking it as dirty. First, if the page is residing in NVM, it copies the page back from NVM into the 
corresponding slot of the internal buffer cache, i.e. \textit{Pg-Buffer}. Second, it undoes the redirection of \textit{PgBufPtr} such that it 
again points to the corresponding slot in the buffer cache and not to the NVM mapped file. This is shown by a black dashed arrow with 
the ``Write'' label in Fig.~\ref{Fig3c}. This way, SE2 ensures that each transaction (or query) updates only its local copy of the page.

In other words, SE1 and SE2 always use the internal PostgreSQL  buffers for write operations, avoiding writes directly into  database files residing in NVM disk. As a result,  data consistency model of PostgreSQL is not violated and transactions are protected from viewing inconsistent data. In summary, SE1 and SE2 operate in the same way as far as write operation is concerned. However, for read operations, SE1 reduces overhead for each miss in internal buffer cache from two copy operations in original PostgreSQL storage engine to one. On the other hand, SE2 reduces this overhead to zero copy operations.

==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}


\noindent System-level evaluation for NVM technologies is challenging due to lack of real hardware. 
Software simulation infrastructures are a good fit to evaluate systems in which NVM is used as a DRAM replacement,
or in conjunction with DRAM as a hybrid memory system. However, when using NVM as a permanent storage replacement, 
most software simulators fail to capture the details of the operating system, and comparisons against traditional disks are not 
possible due to the lack of proper simulation models for such devices. As the authors of PMFS \cite{dulloor2014system} noted, 
an emulation platform is the best way to evaluate such a scenario.

\doublerulesep 0.1pt
\begin{table}[h]
 % \centering
%   \small
  \caption{Test machine characteristics}
  \label{tab:machine}
  \begin{tabular}{@{}ll@{}}
  \toprule
  \textbf{Component} & \textbf{Description} \\ 
  \midrule
  \multirow{2}{*}{Processor}    & Intel Xeon E5-2670 @ 2.60Ghz \\
                                & HT and TurboBoost disabled \\
  \multirow{3}{*}{Caches}       & Private: L1 32KB 4-way split I/D, \\
								& L2 256KB 8-way \\
                                & Shared: L3 20MB 16-way \\
  Memory                        & 256GB DDR3-1600, 4 channels, delivering\\
								& up to 51.5GB/s\\ 
  %\midrule
  OS                            & Linux Kernel 3.11.0 with PMFS support\\  &\cite{githubPMFS,dulloor2014system} \\
  %\midrule
  \multirow{2}{*}{Disk storage} & Intel DC S3700 Series, 400GB, SATA 6Gb/s \\ 
                                & Read 500MBs/75k iops, Write 460MBs/36k \\
                                & iops \\
                                %& Read 851 MB/s, Write 412 MB/s \\
  PMFS storage                  & 224 GB of total DRAM \\%, Read 3.8 GB/s, Write  2.6 GB/s\\  
  \bottomrule
  \end{tabular}
\end{table}


\subsection{Emulation Platform}

We set up an infrastructure similar to that used by the PMFS authors. We first recompile the Linux kernel of our 
test machine with PMFS support. Using the \textit{memmap} kernel command line option we reserve a physically contiguous area of the 
available DRAM at boot-time, which is later used to mount the PMFS partition. In other words, a portion of the DRAM holds the disk 
partition managed by PMFS and provides features similar to those of NVM, such as byte-addressability and lower latency compared to a disk. 
Table~\ref{tab:machine} lists the test machine characteristics. We configure the machine to have a 224GB PMFS partition, leaving 32GB of 
DRAM for normal main memory operation. A high-end SSD is used as regular disk storage.

To fairly evaluate storage engines SE1 and SE2, we compare their performance with two baselines using unmodified PostgreSQL. A similar comparison approach is also adopted by other closely related and complementary works \cite{gao2011pcmlogging,son2017log} using NVM in context of disk-based DBMS as explained in Section~\ref{sec:RelatedWork}.
While comparing with prior work that employs NVM in context of in-memory
DBMS or in from-scratch NVM-aware DBMS designs is out of the scope of this paper, as these systems present different sets of features and target different domains, we do include a qualitative comparison in Section~\ref{sec:RelatedWork}.

The two baselines use unmodified  PostgreSQL 9.5 with the dataset stored in: (i) a regular high-end disk (\textit{disk\_base95}), and (ii) in the PMFS partition (\textit{pmfs\_base95}). The modified storage engines - SE1 and SE2 - are run with the dataset stored on the PMFS partition and are termed \textit{pmfs\_se1} and \textit{pmfs\_se2}, respectively.

%A technological advantage of NVMs over traditional disks is their lower read access latencies. To quantify the performance impact this can have in query executions, we evaluate two baselines using unmodified  PostgreSQL 9.5, (i) with the dataset stored in a regular high-end disk (\textit{disk\_base95}), and (ii) in the PMFS partition (\textit{pmfs\_base95}). In addition, we evaluate the modified storage engines - SE1 and SE2. These are run with the dataset stored on the PMFS partition and are termed \textit{pmfs\_se1} and \textit{pmfs\_se2}, respectively.

Since DRAM read latencies are expected to be similar to projected NVM read latencies \cite{mittal2016survey,arulraj2015let,wang2013low,chang2012limits}, the emulation platform we employed provides good performance estimations. In our experiments, we report wall-clock query execution times as well as data obtained with performance counters using the \textit{perf} toolset. 
\subsection{Workloads}


\begin{figure*}
\centering
\includegraphics[width=\linewidth]{QBDown.eps}
\caption{Execution time breakdown for TPCH queries in traditional DBMS with database stored in disk-storage}
\label{query-breakdown}
\end{figure*}

TPC-H \cite{council2008tpc} is a widely used benchmark and a good representative of decision support system
(DSS) queries. Therefore, to evaluate our proposed SEs, we employ DSS queries from the TPC-H benchmark configured with a scale factor of 100, which leads to a dataset larger than 150GB when adding the appropriate
indexes. Like most data-intensive workloads, these queries are read dominant, which will enable us to draw accurate results from our emulation platform. We report results for 16 of the 22 TPC-H queries since some queries fail to complete under PMFS storage, even when executed with the unmodified PostgreSQL storage engine (i.e. baseline \textit{pmfs\_base95}).

Fig.~\ref{query-breakdown} shows the characterization of the different TPC-H queries in the form of an execution 
time breakdown. The data is collected using a scale factor of 100 with a baseline system that uses a high-end disk as primary storage 
(\textit{disk\_base95}).  The  figure shows two bars: 
functional breakdown (FB) and data movement (DM). FB shows 
the percentage of execution 
time spent across the most relevant database operators, i.e., sequential scan (SeqScan), Sort, Join and all other operations
combined together. DM shows the percentage of execution time spent in the main function performing data reads from 
disk (\textit{mdread}) and also \textit{memcpy} since it is used internally by the kernel to bring data into the application buffers.

As can be seen in the figure, most of the queries are dominated
by sequential scan operations, as expected from read-dominant queries.
This is confirmed by the fact
that most queries spend about 20\% of their execution time bringing
data in from storage to application-level buffers, as shown by
the DM bar.  These overheads are expected to become worse with larger datasets in the future, therefore
lowering the data access latency and avoiding unnecessary data movement is
critical to reduce query execution time. Note that these overheads are due to
data movement operations that can be avoided by reading directly from primary storage with our proposed NVM-aware SEs.


==> pmfs-implications.tex <==
\section{Design Choices}
\label{sec:Implications}
\noindent In this section, we discuss the possible memory hierarchy designs when including NVM in a system. We also discuss the high-level modifications necessary in a traditional disk-optimized DBMS in order to take full advantage of NVM hardware.
\subsection{Memory Hierarchy Designs for an NVM-Based DBMS}

With features of byte-addressability, low latency and high capacity, NVM has the potential to replace traditional disks as well as main memory \cite{chang2012limits}. Fig.~\ref{Fig2} shows different options that might be considered when including NVM into the system. Fig.~\ref{Fig2a} depicts a traditional approach, where the intermediate state - including logs, data buffers, and partial query state - is stored in DRAM to hide disk latencies for data that is currently in use; while the bulk of the relational data is stored in a  disk.

Given the favorable characteristics of NVM over the other technologies, an option might be to replace both DRAM and disk storage 
using NVM (Fig.~\ref{Fig2b}). However, such a drastic change would require a complete redesign of current operating systems and 
application software. In addition, NVM technology is still not mature enough in terms of endurance to be used as a DRAM replacement. 
Hence, we advocate for a platform that still has a layer of DRAM memory, like \cite{kimura2015foedus}, where the disk is completely or partially replaced using NVM, 
as shown in Fig.~\ref{Fig2c} (NVM-Disk).

Using this approach, we can retain the programmability of current systems by still having a layer of DRAM, thereby exploiting DRAM's fast read and write access latencies for temporary data structures and application code. In addition, it allows the possibility to directly access the bulk of the database relational data by using a file system such as PMFS, taking full advantage of NVM technology, which allows the system to leverage NVM's byte-addressability and to avoid API overheads~\cite{huang2014nvram} present in current FSs. Unlike an in-memory DBMS, such a setup does not need large pools of DRAM since temporary data is orders of magnitude smaller than the actual relational database stored in NVM. We believe this is a realistic scenario for future systems integrating NVM, with room for small variations such as NVM alongside DRAM to store persistent temporary data structures, or having traditional disks to store cold data.

\begin{figure} %[!htbp]
\centering     %%% not \center
\subfigure[Traditional design]{\label{Fig2a}\includegraphics[width=27mm]{Fig2a.eps}}
\subfigure[All-in-NVM]{\label{Fig2b}\includegraphics[width=27mm]{Fig2b.eps}}
\subfigure[NVM-Disk]{\label{Fig2c}\includegraphics[width=27mm]{Fig2c.eps}}
\caption{NVM placement in the memory hierarchy of a computing system}
\label{Fig2}
\end{figure}

\subsection{Potential Modifications in a Traditional DBMS}~\label{modList}
Using a traditional disk-based database with NVM storage will not take full advantage of NVM's features. Some important components of the DBMS need to be modified or removed when using NVM as a primary storage. 

\noindent\textbf{Avoid the block level access:} Traditional design of a DBMS uses a disk as a primary storage. Since disks favor sequential accesses, database systems hide disk latencies by issuing fewer but larger disk accesses in the form of a data block~\cite{schindler2002track}. 

Unfortunately, block level I/O causes extra data movement. For example, if a transaction updates a single byte of a tuple, it still needs to write the whole block of data to the disk. On the other hand, block level access provides good data locality.
 
Since NVM is byte-addressable, we can read and write only the required byte(s). However, reducing the data retrieval granularity down to a byte level eliminates the advantage of data locality altogether. A good compromise is to reduce the block size in such a way that the overhead of the block I/O is reduced to an acceptable level, while at the same time the application benefits from some degree of data locality. 
 
\noindent\textbf{Remove internal buffer cache of DBMS:} DBMSs usually maintain an internal buffer cache. Whenever a tuple is to be accessed, first its disk address has to be calculated. If the corresponding block of data is not found in the internal buffer cache, then it is read from disk and stored in the internal buffer cache \cite{debrabant2013anti}. 
 
This approach is unnecessary in an NVM-based database design. If the NVM address space is made visible to a process, then there is no need to copy data blocks. It is more efficient to refer to the tuple directly by its address. However, we need an NVM-aware FS, such as PMFS, to enable direct access to the NVM address space by a process.
 



\subsection{Discussion}
NVM provides the promising features of persistency, like disk storage; and byte-addressability, like DRAM. However, NVMs
have certain limitations such as lower endurance compared to DRAM \cite{arulraj2015let} and a disparity between the read and write latencies \cite{pelley2014memory}. 
Furthermore, different NVM technologies differ from each other in term of these features \cite{arulraj2015let}.

 
A storage engine aiming to improve decision support
system (DSS) queries can be designed by taking advantage
of the common features of persistency and byte-addressability.
Since DSS queries are read dominant and perform a relatively
negligible number of write operations, the design should
not be influenced or sensitive to different endurance and write
latencies found across NVM technologies. Furthermore, NVM technologies
are projected to provide read latencies similar to DRAM \cite{mittal2016survey,arulraj2015let,wang2013low,chang2012limits}.
Therefore, reading data directly from NVM storage should be comparable in terms
of access latency to reading application data stored in DRAM.

 
Usage of NVM as primary storage can also impact
other components of a DBMS besides those mentioned
in Section \ref{modList}. For example, if internal buffers are not
employed and all updates are materialized directly into the
NVM address space then the need and criticality of the redo
log can be relaxed \cite{huang2014nvram}. However, the undo log will still be
needed to recover from a system failure. These important aspects are
out of the scope of this work and we will focus on storage engine modifications.

\begin{figure*}  [!htbp]
\centering     %%% not \center
\subfigure[PostgreSQL storage engine]{\label{Fig3a}\includegraphics[width=38mm]{Fig4.eps}}
\subfigure[Modified storage engine - SE1]{\label{Fig3b}\includegraphics[width=38mm]{Fig5New.eps}}
\subfigure[Modified storage engine - SE2]{\label{Fig3c}\includegraphics[width=38mm]{Fig6New.eps}}
\caption{High level view of read and write memory operations in PostgreSQL (read as ``pg'' in short form) and modified SEs}
\label{Fig3}
\end{figure*}
 


==> related.tex <==
\section{Background}
\label{sec:background}
\noindent In this section, we first describe in detail the properties of NVM technologies, highlighting the implications these might have in the design of a DBMS. We then describe currently available system software to manage NVM. 


\subsection{Characteristics of NVM}
\noindent \textbf{Data access latency:} Read latencies for NVM technologies will certainly be significantly lower than those of conventional disks. However, since NVM devices are still under development, sources quote varying read latencies. For example, the read latency for STT-RAM ranges from 1 to 20ns, and PC-RAM is expected to be around 50ns ~\cite{arulraj2015let,wang2013low,perez2010non}. Nonetheless, read latency of some NVM technologies is expected to be similar to that of DRAM ~\cite{mittal2016survey,arulraj2015let,wang2013low,chang2012limits,arulraj2016write,oukid2014sofort,chatzistergiou2015rewind}, which is typically around 60ns.

PC-RAM and R-RAM are reported to have a higher write latency compared to DRAM, but STT-RAM also outperforms DRAM in this regard ~\cite{arulraj2015let,wang2013low}. However, the write latency is typically not in the critical path, since it can be tolerated by using buffers ~\cite{qureshi2009scalable}.

\noindent\textbf{Density:} NVM technologies provide higher densities than DRAM, which makes them a good candidate to be used as main memory as well as primary storage, particularly in embedded systems~\cite{huang2012register}. For example, PC-RAM provides 2 to 4 times higher density as compared to DRAM~\cite{qureshi2009scalable}. Future NVMs are expected to have higher capacity and better scalability than DRAM \cite{oukid2015instant,chakrabarti2014atlas,zhang2015study,viglas2014write}
, and it is expected to scale to lower technology nodes as opposed to DRAM.

\noindent\textbf{Endurance:} The maximum number of writes a memory cell can withstand is lower for most NVM 
technologies when compared to DRAM ~\cite{qureshi2009scalable,zhou2009durable}. Specifically, PC-RAM, R-RAM, 
and STT-RAM have projected endurances of $10^{10}$, $10^{8}$, and $10^{15}$ respectively;  as compared to 
$10^{16}$ for DRAM ~\cite{arulraj2015let}. On the other hand, NVMs exhibit higher endurance than flash 
memory technologies ~\cite{wang2013low}.

\noindent\textbf{Energy consumption:} Since NVM does not need a refresh cycle to maintain data states in memory cells like a  DRAM, 
they are more energy efficient. A main memory designed using PC-RAM technology consumes significantly lower per access write energy as compared to DRAM~\cite{zhou2009durable}. Other NVM technologies also have similar lower energy consumption per bit when compared to DRAM~\cite{arulraj2015let,perez2010non}.

In addition to the features listed above, NVM technologies also provide byte-addressability like DRAM and persistency like disks. Due to these features, NVMs are starting to appear in embedded and energy-critical devices and are expected to play a major role in future computing systems. Companies like Intel and Micron have launched the 3D XPoint memory technology, which features non-volatility \cite{3DXPoint}. Intel has also introduced new instructions to support the usage of persistent memory at the instruction set architecture (ISA) level~\cite{intel2016architecture}.

\subsection{System software for NVM}

Using NVM as primary storage necessitates modifications not only in application software but also in system software in order to 
take advantage of NVM features. A traditional file system (FS) accesses the storage through a block layer. If a disk is replaced by NVM without any modifications in
the FS, the NVM storage will still be accessed at block level granularity. Hence, we will not be able to take advantage of the byte-addressability feature of NVM. 

For this reason, there have been developments in file system support for persistent memory. Persistent memory file system (PMFS) is an open-source POSIX compliant FS developed by Intel Research~\cite{dulloor2014system,githubPMFS}. It offers two key features in order to facilitate usage of NVM.

First, PMFS does not maintain a separate address space for NVM. In other words, both main memory and NVM use the same address space. This implies that there is no need to copy data from NVM to DRAM to make it accessible to an application. A process can directly access file system protected data stored in NVM at byte level granularity.


Second, in a traditional FS stored blocks can be accessed in two ways: (i) file I/O and (ii) memory mapped I/O. PMFS implements file I/O in a similar way to a traditional FS. However, the implementation of memory mapped I/O differs. In a traditional FS, memory mapped I/O would first copy pages to DRAM~\cite{dulloor2014system} from where an application can examine those pages. PMFS avoids this copy overhead by mapping NVM pages directly into the address space of a process. 
Fig.~\ref{Fig1} from~\cite{dulloor2014system} compares a traditional FS with PMFS.

\begin{figure}
\centering
\includegraphics[width=100mm]{Fig1.eps}
\caption{Comparison of traditional FS and PMFS. ``mmap'' refers to the system call for memory mapped I/O operation. 
``mmu'' is the memory management unit responsible for address mappings}
\label{Fig1}
\end{figure}


